Quantum Gravity on the computer: Impressions of a workshop

Computer simulations allow us to explore non-perturbative phenomena in physics. This has the potential to help us understand quantum gravity. Finding a theory of quantum gravity is a hard problem, but in the last decades many promising and intriguing approaches that utilize or might benefit from using numerical methods were developed. These approaches are based on very different ideas and assumptions, yet they face the common challenge to derive predictions and compare them to data. In March 2018 we held a workshop at the Nordic Institute for Theoretical Physics (NORDITA) in Stockholm gathering experts in many different approaches to quantum gravity for a workshop on "Quantum gravity on the computer". In this article we try to encapsulate some of the discussions held and talks given during this workshop and combine them with our own thoughts on why and how numerical approaches will play an important role in pushing quantum gravity forward. The last section of the article is a road map providing an outlook of the field and some intentions and goalposts that were debated in the closing session of the workshop. We hope that it will help to build a strong numerical community reaching beyond single approaches to combine our efforts in the search for quantum gravity.

==> flowchart.tex <==


%
% \smartdiagram[descriptive diagram]{
%   {Style,{Define shapes, colors, shading,
%           and line styles for nodes and arrows}},
%   {Position, {Place nodes using a matrix,
%               relative or absolute positioning}},
%   {Relation, Insert edges or arrows
%              between selected nodes},
%   {Label, Add labels on edges or arrows}}


  \tikzstyle{mybox} = [draw=black!70, fill=white, very thick,
      rectangle, rounded corners, inner sep=2pt, inner ysep=20pt]
  \tikzstyle{fancytitle} =[fill=black!70, text=white, ellipse]
  \tikzstyle{fancytitle2} =[fill=black!20, text=black, ellipse]
  \tikzstyle{arrow} = [thick,->,>=stealth]
  \tikzstyle{vecArrow} = [thick, decoration={markings,mark=at position
   1 with {\arrow[semithick]{open triangle 60}}},
   double distance=1.4pt, shorten >= 5.5pt,
   preaction = {decorate},
   postaction = {draw,line width=1.4pt, white,shorten >= 14.5pt}]
\tikzstyle{innerWhite} = [semithick, white,line width=1.4pt, shorten >= 4.5pt]

  %

  \begin{tikzpicture}[transform shape, rotate=0, node distance=6cm]

  
  \node (comands) [mybox,xshift=2cm, yshift=0cm]  {%
      \begin{minipage}[t!]{5cm}
         \begin{itemize}
             \item Be honest
             \item Be humble
             \item Do not oversell
         \end{itemize}

      \end{minipage}
      };
  \node[fancytitle] at (comands.north) {The three commandments};

  \node  (asp)[mybox,  xshift= -7cm,yshift=0cm] {%
      \begin{minipage}[t!]{11cm}
         \begin{itemize}
             \item full LORENTZIAN, QUANTUM path integral
             \item connection between different approaches/ fields
             \begin{itemize}
                 \item encourage and support students \\ to work on several approaches
             \end{itemize}
             \item implement and understand symmetries in our theories
         \end{itemize}

      \end{minipage}
      };
       \node (road) [fancytitle2, xshift =-2.5cm, yshift=5cm] {\Huge Destination Quantum Gravity};
  \node[fancytitle] at (asp.north) {Our aspirations};

  \node [mybox,  yshift=-10cm,xshift=-7.5cm] (todo) {%
      \begin{minipage}[t!]{9cm}
         \begin{itemize}
             \item contact with experiment
             \item understand and tame nonlocal effects
             \item compare fixed points
             \item matter couplings
             \begin{itemize}
                 \item CST
                 \item CDT
                 \item what about SUSY?
             \end{itemize}
             \item decoherence functional/ double path integral
         \end{itemize}

      \end{minipage}
      };

  \node (ftodo) [fancytitle] at (todo.north) {Things we need to do};
  
    \node [mybox, xshift=1.5cm,yshift=-7cm] (infra) {%
      \begin{minipage}[t!]{8cm}
         \begin{itemize}
             \item metrics/ goalposts
             \item HPC algorithms
             \item conference series
             \begin{itemize}
                 \item Nordita program
                 \item more computer schools \\to teach students
             \end{itemize}
         \end{itemize}

      \end{minipage}
      };
  \node (finfra) [fancytitle] at (infra.north) {Infrastructure we need to develop};
  \node [mybox,  yshift= -15cm,xshift=1.5cm] (open) {%
      \begin{minipage}[t!]{8cm}
         \begin{itemize}
             \item shared codebase
             \item open source
             \item open data
             \begin{itemize}
                 \item data standards and shared formats?
             \end{itemize}
             \item documentation
         \end{itemize}

      \end{minipage}
      };
  \node (fopen) [fancytitle] at (open.north) {Open Science};

  \draw [vecArrow] (asp)-- (ftodo);
  \draw [vecArrow] (todo)-- (infra);
  \draw [vecArrow] (infra)-- (fopen);
   \end{tikzpicture}

